Learning Bimanual Scooping Policies for Food Acquisition

A robotic feeding system must be able to acquire a variety of foods. Prior bite acquisition works consider single-arm spoon scooping or fork skewering, which do not generalize to foods with complex geometries and deformabilities. For example, when acquiring a group of peas, skewering could smoosh the peas while scooping without a barrier could result in chasing the peas on the plate. In order to acquire foods with such diverse properties, we propose stabilizing food items during scooping using a second arm, for example, by pushing peas against the spoon with a flat surface to prevent dispersion. The added stabilizing arm can lead to new challenges. Critically, this arm should stabilize the food scene without interfering with the acquisition motion, which is especially difficult for easily breakable high-risk food items like tofu. These high-risk foods can break between the pusher and spoon during scooping, which can lead to food waste falling out of the spoon. We propose a general bimanual scooping primitive and an adaptive stabilization strategy that enables successful acquisition of a diverse set of food geometries and physical properties. Our approach, CARBS: Coordinated Acquisition with Reactive Bimanual Scooping, learns to stabilize without impeding task progress by identifying high-risk foods and robustly scooping them using closed-loop visual feedback. We find that CARBS is able to generalize across food shape, size, and deformability and is additionally able to manipulate multiple food items simultaneously. CARBS achieves 87.0% success on scooping rigid foods, which is 25.8% more successful than a single-arm baseline, and reduces food breakage by 16.2% compared to an analytical baseline. Videos can be found at https://sites.google.com/view/bimanualscoop-corl22/home .

==> 3-problem_statement.tex <==
\section{Problem Statement}
\label{sec:problem_statement}

We consider the task of scooping a variety of food items off a plate without any potential food damage or waste. Concretely, we want to successfully transfer the food from the plate to the scooper and also maximize the integrity of the food item, i.e., the weight, after the scooping motion. The food items may vary in geometry and deformabilities. For geometries, we consider variations in size and shape, including thicknesses, roundness, and symmetry. For deformabilities, we consider foods that are brittle (i.e. cashews), compliant (i.e. pasta), and fragile/breakable (i.e. tofu).

\noindent\textbf{Assumptions.} 
We assume access to a plate workspace with a standard $(x,y,z)$ coordinate frame (as shown in Fig.~\ref{fig:fig1}). 
We assume full bimanual access to this plate workspace with the following two mounted tools: \emph{Scooper} and \emph{Pusher} (See Fig.~\ref{fig:exp_setup}). The \emph{Scooper} tool is a plastic spoon mounted at an angle to the robot end effector. Additionally, this tool has a camera mounted for access to angled images $I \in \mathbb{R}^{W \times H \times C}$ of the spoon and surrounding workspace. The \emph{Pusher} tool is a concave barrier that is mounted vertically to the robot end effector\footnote{This design is inspired by antique pushers that were used to push foods into spoons (\url{https://www.etsy.com/market/food_pusher}).}. 

We model the bimanual scooping task as a Markov Decision Process (MDP) $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R})$. 
We observe images $I \in S$ of the unknown food environment and define an action space $\mathcal{A}$ as joint 14-DoF robot actions $(a^s, a^p)$. The visual state space is an RGB image observation space $S \in \mathbb{R}^{W \times H \times C}$. We assume unknown transition dynamics $\mathcal{T}: \mathcal{S} \times \mathcal{A} \xrightarrow{} \mathcal{S}$, an initial state distribution of food configurations $\rho_0$, and a time horizon $T$. We define a reward $\mathcal{R}: \mathcal{S} \times \mathcal{A} \xrightarrow{} \mathbb{R}$ as the weight of the food in the scooper after scooping. We aim to construct a closed loop policy $\pi:\mathcal{S} \xrightarrow{} \mathcal{A}$ to maximize the expected reward by successfully scooping a set of varied foods.




     


==> 4-carbs.tex <==
\section{\algname{}}
\label{sec:methods}
\algabbr{} learns to scoop a variety of food items by employing a bimanual scooping primitive combined with a learned system for recognizing high-risk foods and avoiding breakage failures (Fig.~\ref{fig:fig1}).
In this section, we introduce a stabilizing action parameter to adjust the pusher and scooper to deformable and breakable foods. We also present the learned vision-based models that identify food fragility and breakage-imminent states, where the food is exactly between the pusher and scooper but not yet squeezed to cause breakage. Given this visual feedback, \algabbr{} is able to scoop a wide range of food items without breakage.

Given an overhead image observation $I_0$, \algabbr{} starts by identifying the food position in the initial environment state $s_0$. To do this, we learn a segmentation model $s:\mathbb{R}^{1280 \times 720 \times3} \xrightarrow{} \mathbb{R}^{1280 \times 720}$ to obtain a food mask and food center position $(x_f, y_f)$ from the initial image $I_0$. 
The scooper and pusher are initially centered around this food center along the a fixed pushing axis.
Next, \algabbr{} executes the parameterized bimanual scooping primitive in three phases: (1) \emph{Pushing}, (2) \emph{Scooping}, and (3) \emph{Transfer}. 

\noindent\textbf{Pushing.} During \emph{Pushing} phase, both the pusher and scooper move towards each other along the $x$-axis until they meet at some $(x_f+d', y_f)$. The pusher travels a distance of $d+d'$ while the scooper travels $d-d'$.
% this phase has two bimanual stabilization strategies
This phase utilizes two bimanual stabilization strategies: an angled pusher and the pushing motion. First, the pusher is angled at some angle $\theta$ off the vertical, rather than orthogonal to the plate. This stabilizes the food position by encouraging the food to slide or roll into the scooper at the end of pushing when the two arms meet. The second stabilization strategy is the pushing motion of the pusher. This motion moves the food towards the scooper and pins the food against the concave pusher surface, which promotes centering the food position during movement into the entrance of the spoon.
% one of these stabilization strategies is parameterized
We adapt the pushing motion strategy with a stabilizing action parameter $\alpha \in [0, 1]$, which represents a proportion of the distance traveled by the arms and length of the Pushing phase. When $\alpha = 0$, both arms are stopped and move to the Scooping phase. When $\alpha = 1$, we execute the full Pushing phase with the pusher traveling a distance of $d+d'$. When scooping, it is critical to adapt $\alpha$ to prevent breakage failures of fragile foods.

\noindent\textbf{Learning to Stabilize.} It is nontrivial to select an $\alpha$ value given only an initial observation $I_0$, because varied food dynamics can dictate the need for different $\alpha$ values even for the same food item. For example, when scooping two identical pieces of tofu, the food items may slide or roll on the plate differently due to food interactions with the plate or slight robot imprecision.
We learn two classifiers to select appropriate $\alpha$ values for our dynamic stabilizing policy.
We first learn a risk classifier $r:\mathbb{R}^{1280 \times 720 \times3} \xrightarrow{} [0,1]$ that identifies an initial food image $I_0$ as ``Robust" or ``Fragile". If the food is ``Robust", \algabbr{} uses $\alpha = d+d'$ for maximum stabilization (pushing) of the food, since the food is not in danger of breaking. If the food is ``Fragile", our policy adjusts $\alpha$ with visual feedback to prevent breakage. We learn a failure classifier $f:\mathbb{R}^{1280 \times 720 \times 3} \xrightarrow{} [0,1]$ that identifies breakage-imminent states where the food item is in contact with both the pusher and scooper, but not yet squeezed to cause breakage. For fragile, high-risk foods, \algabbr{} uses this classifier to servo for breakage-imminent states, and terminates the Pushing phase early, effectively decreasing $\alpha < 1$. In practice, we instantiate these classifiers with two ResNet34 models~\todo{cite} trained on a hand-labelled food fragility and food breakage dataset respectively.

\noindent\textbf{Scooping and Transfer.} After the Pushing phase, we assume \algabbr{} has successfully manipulated the food item into the scooper and move to the \emph{Scooping} phase. In this phase, we rotate the scooper up about the $y$ axis to ``scoop" the food into the bowl of the spoon. During the Scooping phase, \algabbr{} employs a third bimanual stabilizing strategy where the pusher moves up along the $z$ axis with the scooper as it rotates. This strategy prevents foods from falling out of the scooper, especially food items that are in unstable poses in the spoon. Lastly, \algabbr{} finishes with the \emph{Transfer} phase by moving the pusher away from the scooper and rotating the scooper towards an end use to prepare for feeding.

% - overview of method
%     - we first find the food position on the plate with segmentation
%     - we then move to scoop our food in three phases: pushing, scooping, and transfer
%     - Pushing. here we put the two arms on either side of the food position and push together. *pusher is angled slightly.
%         - this is one of the bimanual stabilizing motions, which is cool.
%             - prevents the foods from rolling away.
%             - pusher is angled slightly to encourage foods to roll into the scooper.
%         - this is adjustable depending on the food. how much are we pushing? "stabilizing action parameter"
%     - Learning to Stabilize. how do we adjust this stabilizing parameter?
%         - first we train a classifier to identify high-risk foods (deformable, breakable).
%         - if we are scooping a high-risk food, we use visual feedback in the form of a breakage failure classifier to servo for when to stop the first phase (pushing). This effectively adjusts our stabilizing action parameter.
%         - now we have our food item in our scooper without it breaking. continue with primitive:
%     - Scooping. here we put the pusher arm at the edge of the scooper as it scoops and follows it up. 
%         - this is another stabilizing motion. 
%             - prevents foods from falling out of scooper during scooping if in an unstable pose. 
%         - this also adjusted with the same "stabilizing action parameter". the pusher just starts following the scooper up from wherever it stops.
%     - Transfer. here we move the pusher away from the scooper and rotate the scooper away from the plate workspace to prepare for bite transfer for feeding a human. 
    
    


==> 4-methods.tex <==
\section{\algname{}}
\label{sec:methods}

- overview of method
    - we first find the food position on the plate with segmentation
    - we then move to scoop our food in three phases: pushing, scooping, and transfer
    - Pushing. here we put the two arms on either side of the food position and push together. *pusher is angled slightly.
        - this is one of the bimanual stabilizing motions, which is cool.
            - prevents the foods from rolling away.
            - pusher is angled slightly to encourage foods to roll into the spoon.
        - this is adjustable depending on the food. how much are we pushing? "stabilizing action parameter"
    - Learning to Stabilize. how do we adjust this stabilizing parameter?
        - first we train a classifier to identify high-risk foods (deformable, breakable).
        - if we are scooping a high-risk food, we use visual feedback in the form of a breakage failure classifier to servo for when to stop the first phase (pushing). This effectively adjusts our stabilizing action parameter.
        - now we have our food item in our spoon without it breaking. continue with primitive:
    - Scooping. here we put the pusher arm at the edge of the spoon as it scoops and follows it up. 
        - this is another stabilizing motion. 
            - prevents foods from falling out of spoon during scooping if in an unstable pose. 
        - this also adjusted with the same "stabilizing action parameter". the pusher just starts following the spoon up from wherever it stops.
    - Transfer. here we move the pusher away from the spoon and rotate the spoon away from the plate workspace to prepare for bite transfer for feeding a human. 
        

\algabbr{} learns to scoop a variety of food items by employing a bimanual scooping primitive combined with a learned system for recognizing high-risk foods and avoiding breakage failures (Fig.~\ref{fig:fig1}).
In this section, we will first define a bimanual action that controls the pusher and spoon. Next, we will present the learned components that identify the deformability of food items and breakage-imminent states. Given this visual feedback, \algabbr{} should be able to scoop a wide range of food items without breakage.

\subsection{Bimanual Scooping Primitive}
% \noindent\textbf{Bimanual Scooping Primitive.}
\todo{rewrite to use action space from problem statement}
% \todo{figure system overview}
% - talk about past primitives
% - emphasize that the pusher moves up with the spoon
%     - it helps foods roll into the spoon when theyre on the edge
%     - it helps unstable geometries stay on the spoon as we scoop up (eg snowpeas)
% - angle the pusher instead of vertical because that is helpful for getting foods to roll into the spoon rather than get stuck between then pusher and the spoon (eg cashews)
% - we tried different spoon angles but it doesn't help
% talk about the single arm primitive and their disadvantages
% Single-arm dynamic scooping primitive, which uses the robot arm end-effector to move and rotate the mounted spoon with the action space $A_s = (dy_s, \Delta \gamma_s, \Delta \beta_s)$, can already acquire food items from the plate. However, previous single-arm primitives are limited to relatively homogeneous geometries and deformability and therefore, not generalizable to a variety of food in the real world. For example, it is difficult to scoop round and rolling items, i.e., peas and blueberries, with a single arm because there are no barriers to stop the chasing. 

% propose the bimanual primitive and motivates the pusher design
To address this issue of the single-arm primitive, we define a bimanual scooping primitive $(A_s, A_p)$ where $A_p = ( dy_p, dz_p, \Delta \gamma_p )$ and use an additional robot arm to control the pusher. Specifically, the designed pusher is supposed to group food from the edge to the center, to work as a barrier to prevent the chasing of food items and most importantly to stabilize them and forestall potential dropping when the spoon rotates. To better serve these purposes, we design a concave pusher in Figure \ref{fig:exp_setup} that is suited to the degree of curvature of the front end of the spoon.

% talk about past baseline primitive we have tried and their cons, e.g. push on the table, nominal 
% talk about our primitve in details about how the motion of the two arms are defined and how they are able to acquire the food, we tried different spoon angles
\todo{measure these specific distance and angle}
To achieve an efficient, generalizable dual-arm bite acquisition system, we have designed a bimanual scooping primitive that incorporates the three processes of pushing $(T=1)$, scooping $(T=2)$ and transferring $(T=3)$ with our proposed pusher and the spoon. The whole process of the primitive is illustrated as follows. When $T=0$, we set the spoon action as $a_{s,0} = (xx, 30, 0)$ and set pusher action as $a_{p,0} = (-xx, 0, 0)$ as the initial start position for pusher and spoon. When $T=1$, the spoon action $a_{s,1} = (xx, 0, 0)$ and the pusher action $a_{p,1} = (-xx, 0, r)$ are given to make them push towards each other, thus grouping food items and roll them into the spoon. At time step $T=2$, action $a_{s,2} = (xx, rr, 0)$ and action $a_{p,2} = (yy,zz, rr)$ are given to the spoon and the pusher to make the pusher tilt back and the spoon rotate to flat position. In our last step (T=3), we give action $a_{p,3} = (-xx,0, 0)$ to the pusher to move that away from the spoon and $a_{s,3} = (0,0,rr)$ to the spoon so that it would rotate and test the stability of acquired food in the spoon. % specific details of each process 

The success of food acquisition is sensitive to the the starting rotation angle of the spoon and the pusher (T=0). The angle of the spoon and the pusher is not too large. Otherwise, it will break the constraints of the two arms and cause the conflict of two arms. At the same time, the angle is not supposed to be too small, either. The key intuition behind this is that the front end of the spoon should be low enough to touch the plate so that food items will roll easily into the spoon instead of being caught between the space between the spoon and the plate. The pusher is also required to be in a proper angle so that it adds a rolling motion to both $x$ and $z$ axes to get food items into the spoon. 

Then, during scooping (T=2), the spoon would rotate along the x-axis of the robot arm from the mounted point to be parallel to the plate and the pusher would move up and tilt back to follow the motion of the spoon. Once the pusher and the spoon reaches their goal positions, the pusher will move away from the spoon and the spoon will rotate along the z-axis of the workspace to test the stability of food items in the spoon. The entire motion primitive of the two arms is demonstrated in Figure \ref{fig:fig1}.

\subsection{Learning to Stabilize}
% \noindent\textbf{Learning to Stabilize.}
\label{subsec:learning}
% - let's keep things more general
% - segmentation
%     - dataset
%     - model
% - we should stop early bc that is helpful
%     - its helpful to stop early in some cases, but hurtful to stop early in others.
%     - when is it hurtful to stop early? foods with similar traits (high-risk foods) all have similar failures that stopping early can solve. let's use that idea.
% - how do we know when to stop early and how early to stop?
% - let's learn to recognize when it is helpful to stop early (when foods are high-risk), and then learn when to stop
% - refer to figure
% - classifying 
%     - resnet to classify
%     - dataset size
%     - augment 7x
% - servoing
%     - resnet to classify
%     - small images
%     - hand label 30 rollouts per fragile food
%     - augment 7x
%     - we should talk about why we do not use hpatic as a sensing mode for this servoing classifier. it might even be helpful to include plots of the force sensing during breakage as a figure in the appendix to show that the breakage failure reading on the force sensor is too subtle to detect. therefore we use vision and only and also bypass the need for an expensive f/t sensor
With our bimanual scooping primitive, our system is already able to successfully acquire a set of non-fragile food. However, the designed primitive is not ideal for fragile food because without considering the deformability, the direct pushing of food into the spoon would lead to breakage of some fragile food, i.e., tofu, cheesecake and jello cube. Therefore, a natural modification to our system is to stop the pusher earlier if the food is fragile so that less force would be applied. Even though the early stop of the pusher may not get fragile food fully into the spoon, the following scooping motion would carefully rotate and cover the food until the food is fully in the spoon parallel to the table.

Therefore, to further extend the generalization of our system, we have a segmentation model to visually identify the food on the plate in the first part of our full system pipeline before the execution of actions because we want to align the pusher and spoon to be in a line with food. Then, between $T=0$ and $T=1$, we use our trained Deformability Classifier to distinguish the food property. If the food is classified as fragile, the trained Breakage Classifier will predict the breakage-imminent state during $T=1$, the pushing process, to stop the motion earlier. Our data-driven approach also enables the Breakage Classifier to generalize to unseen fragile foods.

The following section will discuss the segmentation model and classifiers in details.



\noindent\textbf{Segmentation Model}
We now develop a Segmentation Model to predict the segmentation mask of a variety of food items in our workspace. To build a generalizable model that is not biased by food types or various lighting conditions. We augment the dataset images and balance the number of images per food class. The augmentation applies rotation, translation and flipping as well as the change in color, e.g., adding noise in hue and saturation, increasing linear contrast, to images. Details of augmentation are listed in the Appendix \todo{add augmentation details to appendix}. We also subtract the images with the ground-truth clean background to get a clear segmentation mask for training. The input of our model is a RGB image $I\in\mathbb{R}^{1280\times720\times3}$. After cropping and resizing, we input the image $\hat{I}\in \mathbb{R}^{640 \times 480\times3}$ through a ResNet64\cite{he2016deep} model integrated with Feature Pyramid Network \cite{lin2017feature} and the activation function of sigmoid is applied to make the output lie in the range of $(0,1)$. The final mask $M \in {\{0,1\}}^{640\times480}$ is further cropped to \todo{(xx, yy)} exclude any outliers from the edges of the plate and the spoon. With the cropped mask, the system is able to locate pixel location of the center of the food item by averaging over all the pixels in the mask. Moreover, with a depth image $I^d\in (0.3,3)^{1280\times720\times1}$ captured from the same camera position, we can project the 2D pixel location $(x^p, y^p)$ to the 3D position $(x^c,y^c,z^c)$ in the camera frame. After camera calibration, the 3D food position $(x^c, y^c, z^c)$ is translated into location $(x^w, y^w, z^w)$ in the world frame. Before time step T=0, we set the initial position of the spoon as $s_s = (x^w, y^w + d, z_w)$ and the position of the pusher as $s_p=(x^w , y^w-d, z^w)$ where $d$ is the distance offset of \todo{xx} millimeters.

\noindent\textbf{Fragility Classifier} Let $l^c \in L^c = {\{l | l < 15, l\in \mathbb{N}^*\}}$ be the number of food category label, $l^f \in L^f = \{0,1\}$ be the label of food deformability, where 0 stands for fragile food and 1 stands for robust food. We manually map $l^c$ to $l^f$ given the food properties and only tofu, cheesecake and red jello are labelled as the fragile food. In total, the food dataset has $40 \times 15=600$ images of different types and positions. We also apply the same augmentation for the RGB image $I\in\mathbb{R}^{1280\times720\times3}$ as segmentation model and use ResNet34 \cite{he2016deep} as our model for the prediction of the binary label $\hat{l}^f$, where $\hat{l}^f = f(I)$ and $f$ is our classifier model. During the training, we use Binary Cross Entropy Loss to guide the update of the model. Suppose our dataset $D$ has $N$ samples, the BCE Loss is formalized as below.
\begin{equation}
    L = \frac{1}{N}\sum_{i= 1, d_i\in D}^N  ( l^f_i \times log(f(d_i))  + (1- l^f_i)\times log(1-f(d_i))
\end{equation}
After validating our Fragility Classifier on our food dataset, we use it before time step T=0 and only apply the following Breakage Classifier for foods that are classified as fragile label ($l^f=0)$ during the pushing process at time step T=1. The threshold we set for classification is $0.6$.

\noindent\textbf{Breakage Classifier} Similar to the Fragility Classifier, we use the same augmentation to the images in the food dataset and train a ResNet34 \cite{he2016deep} to predict the breakage-imminent state. Let $l^b \in L^b = \{0,1\}$ detonates the label for the breakage-imminent state where 0 stands for breakage-free state and 1 stands for state that is prone to break in the next step. In the dataset, we have 20 trials of tofu scooped with bimanual primitive and we record all the frames in the pushing process and manually label each frame as break-free or break-imminent. Trained with the same BCE Loss, we set the model prediction threshold to be 0.98 and it generalizes well to unseen fragile food, e.g., cheesecake and red jello.

